HiClass: a Python library for local hierarchical classification compatible with scikit-learn

HiClass is an open-source Python library for local hierarchical classification entirely compatible with scikit-learn. It contains implementations of the most common design patterns for hierarchical machine learning models found in the literature, that is, the local classifiers per node, per parent node and per level. Additionally, the package contains implementations of hierarchical metrics, which are more appropriate for evaluating classification performance on hierarchical data. The documentation includes installation and usage instructions, examples within tutorials and interactive notebooks, and a complete description of the API. HiClass is released under the simplified BSD license, encouraging its use in both academic and commercial environments. Source code and documentation are available at https://github.com/scikit-learn-contrib/hiclass.

==> coverletter.tex <==
% !TEX program = pdflatex
\input{coverletter_preamble.tex}

\usepackage{xurl}

\usepackage[autostyle]{csquotes}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Dr. Gramfort and anonymous reviewers,

We are pleased to submit a revised version of our manuscript titled ``HiClass: a Python library for local hierarchical classification compatible with scikit-learn''. We have carefully addressed the comments from reviewer \#1, including:

\begin{itemize}
    \item Addressing the request to perform cross-validation and hyperparameter tuning to avoid bias.
    \item Improving the documentation to explain the binary policies for the local classifier per node.
    \item Adding support for the parameter sample\_weight in the fit methods of all classifiers.
\end{itemize}

A detailed point-by-point response to the reviewer's concerns is given in a separate document.

\bigskip

Best regards,

\medskip

Prof. Dr. Bernhard Renard (Hasso Plattner Institute)\\
F\'abio Miranda (Hasso Plattner Institute)\\
Niklas Köhnecke (Hasso Plattner Institute)

\newpage

\textbf{Action editor comments}

\begin{displayquote}
\textit {Dear authors,}

\textit{you work has now been reviewed. The remaining important comment concerns the use of better tuned parameters. Please address this point in a convincing manner and the paper should be good to go.}
\end{displayquote}

Thank you for considering our manuscript and allowing us to submit a revised version. We addressed the reviewer's concerns regarding avoiding bias, code and documentation, and modified the manuscript and library accordingly, as outlined in the responses to the reviewers below.

\bigskip

\textbf{Reviewer \#1}

\begin{displayquote}
\textit{The manuscript and the code have both been significantly improved compared to the last version, and the given example clearly shows how the new proposed models compare with existing ones.}

\textit{From that perspective, as a user, I would certainly be convinced to try it out.}
\end{displayquote}

Dear reviewer \#1, we thank you very much for carefully reading our manuscript, benchmark source code and documentation. We are also extremely grateful for the words of encouragement and the critical feedback for improvements. We have attentively addressed all your comments, as summarized below.

\begin{displayquote}
\textit{However, the work doesn't apply any hyper parameter tuning on the data at all, and that doesn't seem fair. It could be the case that the default hyper parameters of the proposed models happen to be more suitable for the dataset against which the benchmark is run. A simple cross\_val\_score would be an improvement to the existing benchmark.}
\end{displayquote}

We completely agree with this. Hence, in order to reduce bias, 5-fold cross-validation and hyperparameter tuning with Optuna are now performed in the benchmark. Unfortunately, the search space is rather small due to the task being quite time-consuming, however, we specifically selected hyperparameters that we believe would be more beneficial to improve the F-score. If you would like us to test specific hyperparameter combinations or update anything else in the benchmark to make it less biased we are happy to do so according to suggestions.

Furthermore, the repository now contains results obtained from the hyperparameter tuning experiments, which are available at \url{https://github.com/mirand863/hiclass/tree/main/benchmarks/consumer_complaints/results}. Additionally, the supplementary material contains detailed explanation about the experiments and a results figure without hyperparameter tuning for comparison. Overall, the F-scores improved after the cross-validation and hyperparameter tuning.

\begin{displayquote}
\textit{Additional improvements which would be nice to have, are about enhancements on the documentation and the API, for instance, LocalClassifierPerNode's documentation includes:}

    binary\_policy (str, default="siblings") – Rules for defining positive and negative training examples.

\textit{Without explaining what other possible rules are and what they exactly do.}
\end{displayquote}

Thank you for noticing and pointing this mistake! The missing policies were added to the documentation in two locations:

\begin{itemize}
    \item The constructor for the local classifier per node at \url{https://hiclass.readthedocs.io/en/latest/api/classifiers.html#LocalClassifierPerNode.LocalClassifierPerNode.__init__};
    \item Formal definition about the training policies available on \url{https://hiclass.readthedocs.io/en/latest/algorithms/training_policies.html}.
\end{itemize}

\begin{displayquote}
\textit{On the API side, the fit methods don't accept any other fit parameters which can be forwarded to the underlying estimators, e.g. sample\_weight.}
\end{displayquote}

Thank you for the great suggestion! We have added the sample\_weight parameter as requested. However, we could not find in scikit-learn's documentation and source code any other parameter that could possibly be provided to the fit method. If we missed any parameters that we are not aware of, please let us know.

\begin{displayquote}
\textit{Thanks for all the work!}
\end{displayquote}

Thank you once more for the helpful feedback! The suggestions certainly improved the manuscript, documentation and library.

\bigskip

\textbf{Reviewer \#2}

\begin{displayquote}
\textit{First, I would like to mention the very substantial amount of work done by the authors since the
first submission.}

\textit{Many changes have been made, including:}
\begin{itemize}
    \item \textit{the package has been moved to GitHub,}
    \item \textit{the paper includes supplementary materials with more details on the different hierarchical classification strategies,}
    \item \textit{continuous integration is now performed using GitHub actions on all three major operating systems,}
    \item \textit{code coverage is now reported online using codecov and is higher,}
    \item \textit{the documentation is now much more exhaustive, with:}
    \begin{itemize}
        \item \textit{a “getting started” section (installation instructions and simple examples, including links to Google Colab examples),}
        \item \textit{much more information about the algorithms for which implementations are provided,}
        \item \textit{a full documentation of the public API, including the metric functions.}
    \end{itemize}
\end{itemize}
\textit{I think that the package is now much more complete, with the necessary basis for future development being setup.}

\textit{All my main concerns have been addressed.}

\end{displayquote}

Dear reviewer \#2, your positive assessment and careful review of our manuscript, supplementary materials, source code and documentation is greatly appreciated. We also believe the library acquired all the foundations for future development after we addressed your concerns in the previous iteration.

\end{document}
